A survey on modelling of infectious disease spread and control on social contact networks

Infectious diseases are a significant threat to human society which was over sighted before the incidence of COVID-19, although according to the report of the World Health Organisation (WHO) about 4.2 million people die annually due to infectious disease. Due to recent COVID-19 pandemic, more than 2 million people died during 2020 and 96.2 million people got affected by this devastating disease. Recent research shows that applying individual interactions and movements data could help managing the pandemic though modelling the spread of infectious diseases on social contact networks. Infectious disease spreading can be explained with the theories and methods of diffusion processes where a dynamic phenomena evolves on networked systems. In the modelling of diffusion process, it is assumed that contagious items spread out in the networked system through the inter-node interactions. This resembles spreading of infectious virus, e.g. spread of COVID-19, within a population through individual social interactions. The evolution behaviours of the diffusion process are strongly influenced by the characteristics of the underlying system and the mechanism of the diffusion process itself. Thus, spreading of infectious disease can be explained how people interact with each other and by the characteristics of the disease itself. This paper presenters the relevant theories and methodologies of diffusion process that can be used to model the spread of infectious diseases.

==> 2_chap_backg.tex <==
\textbf{\chapter{Overview and Relevant Works}}
Diffusion processes are used to explain dynamic phenomena evolving on networked systems. In a diffusion process, contagious items spread out in the networked system through the inter-node interactions. The evolution behaviours of the diffusion process are strongly influenced by the characteristics of the underlying system and the mechanism of the diffusion process itself. Thus, understanding the characteristics of the underlying system and their impacts on the diffusion process have recently attracted intensive research. Current research on diffusion processes assumes that the sender node and the receiver node are concurrently active to participate in transferring contagious items. However, there are several diffusion processes such as infectious disease spreading and message dissemination in Online Social Networks (OSN) where interacting nodes do not require to be active concurrently to create infectious items transmission links. In these diffusion processes, the contagious items can transmit even with delayed interaction between contagious items and receiver nodes. Thus, these diffusion processes occur through both direct and indirect interactions. This chapter discusses the current literature of diffusion studies and describes the applicability of methods and theories for diffusion dynamics with indirect interactions. 

\input{2.1_chap_diff}
\input{2.2_chap_idis}
\input{2.3_chap_net}
\input{2.4_chap_pro}
\input{2.5_chap_con}

			

